Stereo-Talker: Audio-driven 3D Human Synthesis with Prior-Guided Mixture-of-Experts

This paper introduces Stereo-Talker, a novel one-shot audio-driven human video synthesis system that generates 3D talking videos with precise lip synchronization, expressive body gestures, temporally consistent photo-realistic quality, and continuous viewpoint control. The process follows a two-stage approach. In the first stage, the system maps audio input to high-fidelity motion sequences, encompassing upper-body gestures and facial expressions. To enrich motion diversity and authenticity, large language model (LLM) priors are integrated with text-aligned semantic audio features, leveraging LLMs' cross-modal generalization power to enhance motion quality. In the second stage, we improve diffusion-based video generation models by incorporating a prior-guided Mixture-of-Experts (MoE) mechanism: a view-guided MoE focuses on view-specific attributes, while a mask-guided MoE enhances region-based rendering stability. Additionally, a mask prediction module is devised to derive human masks from motion data, enhancing the stability and accuracy of masks and enabling mask guiding during inference. We also introduce a comprehensive human video dataset with 2,203 identities, covering diverse body gestures and detailed annotations, facilitating broad generalization. The code, data, and pre-trained models will be released for research purposes.

==> fig/f1.tex <==


\begin{figure}
    \centering
    \includegraphics[width = 0.47\textwidth]{img/video_driven3.png}
    \caption{Comparisons with video generation methods.}
    \label{fig:video_driven}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width = 1\textwidth]{img/vloggerAdd3.png}
    \caption{More visualization comparisons with Vlogger.}
    \label{fig:vlogger_add}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width = 0.47\textwidth]{img/face_RD2.png}
    \caption{Comparisons with talking head generation methods}
    \label{fig:compare_face}
\end{figure}

==> intro_bk0808.tex <==

\section{Introduction}
The automatic synthesis of lifelike videos depicting a 3D speaking individual, driven by audio input and a single reference image, presents a groundbreaking advancement with profound implications across a myriad of domains, including film-making, augmenting human-computer interaction paradigms, and virtual reality.
%Intuitively, the key factors in audio-driven human synthesis are 1) the generation of high-fidelity bodily movements and facial expressions, characterized by precise lip synchronization, vivid expression, and a broad range of body gestures; 2) the capability to produce photo-realistic and temporally consistent talking video.
Intuitively, the pivotal aspects of audio-driven human synthesis comprise: 1) generating high-fidelity bodily movements and facial expressions, including precise lip synchronization, vivid emotions, and a broad range of gestures; 2) the capacity to yield photo-realistic and temporally coherent talking videos; and 3) supporting the continuous view-point control and 3D consistency.

%, and this innovation holds the potential to dramatically transform industries like film-making, augmenting human-computer interaction paradigms, and virtual reality.

%The automatic synthesis of a lifelike video depicting a speaking individual, driven solely by provided audio and a single reference image, presents a groundbreaking advancement with profound implications across a myriad of domains. This technology stands to revolutionize sectors such as film production, enhancing human-computer interfaces, and enabling ultra-realistic telepresence experiences.

% 0518
%Early attempts towards this objective normally overlook appearance details, concentrating predominantly on the creation of human skeleton sequences that align with guiding audio through a search-and-connect manner \cite{cassell1994animated, huang2012robot, marsella2013virtual}.
% 0518

%Early attempts towards audio-driven human synthesis normally overlook body parts, concentrating predominantly on the creation of mouth region that align with guiding audio \cite{prajwal2020lip, song2022talking}. Benefit from the progress of face reenactment methods \cite{bounareli2023hyperreenact, hsu2022dual}, generating 
%full head talking videos based on a single portrait image have been widely explored \cite{yu2023talking, zhang2023sadtalker, shen2023difftalk}.  
Early attempts towards addressing audio-driven human synthesis often concentrate on the generation of mouth region coherent with guiding audio signals, neglecting other body parts \cite{prajwal2020lip, song2022talking, sun2022masked, cheng2022videoretalking}. Benefiting from the progress of face reenactment methods \cite{bounareli2023hyperreenact, hsu2022dual}, producing full-head talking videos derived from single portrait images has been widely explored \cite{yu2023talking, zhang2023sadtalker, shen2023difftalk}.
%In pursuit of high-quality visual realism, researchers \cite{liu2022audio, he2024co, liu2023moda} further propose unified frameworks designed to synthesize co-speech gesture videos under audio guidance. 
% Corona et al. \cite{corona2024vlogger} further present a method capable of generating talking human videos using an audio clip and just a single portrait image by first predicting body motion and facial expressions from audio and then render them based on human video generation methods \cite{hu2023animate, zhang2023adding}.
% However, it simply hypothesizes that human body movements are mainly correlated to low-level rhythmic audio features, while high-level semantic content has been proven to be essential in generating diverse body gestures \cite{ao2022rhythmic, liu2022disco}.
Corona et al. [\citeyear{corona2024vlogger}] further present an approach that leverages a single portrait image and an audio clip to synthesize talking human videos. This is achieved by firstly mapping audio input to corresponding body gestures and facial expressions, followed by rendering these predicted motions utilizing advanced human video generation methodologies \cite{hu2023animate, zhang2023adding}. 
Nonetheless, it posits that human body movements are mainly correlated to low-level rhythmic audio features. In contrast, recent studies \cite{ao2022rhythmic, liu2022disco} have emphasized the critical role of high-level semantic content in enriching and diversifying body gesture generation. Consequently, this oversimplified hypothesis leads to a restricted variety in the produced motion sequences.
Moreover, existing human video generation approaches \cite{hu2023animate, xu2023magicanimate} normally incorporate temporal attention modules and motion modules to address the temporal instability of diffusion-based models \cite{rombach2022high}. Nonetheless, these strategies often prove insufficient as they uniformly render the entire images, thereby overlooking the unique characteristics inherent in distinct segments of human images.
% Moreover, existing human video generation approaches \cite{hu2023animate, xu2023magicanimate} often integrate the temporal attention module and motion module to deal with temporal instability inherent in stable diffusion based model \cite{rombach2022high}.
% However, such strategies often fall short as they render entire images uniformly, overlooking the distinct characteristics inherent in human image segments. 
%This oversight may lead to instability within the generated outputs.
%Despite these substantial achievements, most methods simply hypothesize that human body movements are mainly correlated to rhythmic and percussive elements of speech. This has led to a reliance on hand-crafted low-dimensional rhythm-centric features for generating skeleton sequences while ignoring high-dimensional semantic features and corresponding prior knowledge, inadvertently curtailing the breadth and depth of expressiveness achievable in the synthesized gestures.
%, thereby marking a significant leap forward in personalized and immersive audiovisual synthesis.

%Early attempts to achieve this goal leave the appearance information ignored and mainly focus on generating human skeleton sequences coherent with driven audio in a searching-and-connecting manner\cite{cassell1994animated, huang2012robot, marsella2013virtual}.
%Benefiting from the emergence of large-scale co-speech datasets, recent progress has seen achieved by employing diverse deep neural network architectures to model the correlation between speech and gesture \cite{ginosar2019learning, yoon2020speech, yi2023generating, zhu2023taming}.
%, including Generative Adversarial Networks (GANs), Variational Autoencoders (VAEs), and Diffusion models. 
%These methodologies have been extensively investigated to elucidate the intricate mapping between low-dimensional audio characteristics, such as Mel Frequency Cepstral Coefficients (MFCCs), and corresponding motion patterns. This research surge is fueled by the prevailing theory that human motor behaviors are intrinsically linked to the rhythmic aspects of speech, thereby necessitating models that can capture these subtleties in the auditory domain and translate them into expressive bodily gestures.
%Benefiting from the development of large-scale co-speech datasets, methods based on various deep neural networks like GAN, VAE, and Diffusion models have been widely explored to learn the mapping relationship between low-dimensional audio features like MFCC and motion sequences, since the hypothesis that human motions are mainly related with rhythm.
% Based on the hypothesis that human motions are mainly related with rhythm, researchers explore to generate motion from low-dimensional audio features like MFCC based on GAN \cite{ginosar2019learning, yoon2020speech}, VAE \cite{yi2023generating}, and Diffusion \cite{zhu2023taming}.
% To improve the visualization performance, \cite{liu2022audio, he2024co} propose a unified framework to generate audio-driven co-speech gesture videos. Enric 
% \textit{et.al} \cite{corona2024vlogger} further propose to generate talking human based on an audio and a single portrait image.
%  has significantly propelled advancements in the field

% 0518
%The recent rise of large-scale co-speech datasets \cite{zhang2021flow, porgali2023casual}, coupled with the strategic deployment of various deep neural network architectures \cite{kingma2014auto, ho2020denoising, goodfellow2014generative}, has significantly accelerated progress in this domain, which not only enhanced the vividness of motion by learning the correlation between spoken content and corresponding gestures \cite{ginosar2019learning, yoon2020speech, zhu2023taming}, but also enriched expressiveness by extending predictive capabilities from focusing solely on body gestures to encompassing facial landmarks as well \cite{yi2023generating, liu2023emage}.
% 0518

%With the recent rise of large-scale co-speech datasets and the application of various deep neural network architectures \cite{ginosar2019learning, yoon2020speech, yi2023generating, zhu2023taming}, this field has been significantly propelled advancements not only in motion vivid by modeling the correlation between speech content and accompanying gestures, but also in expressive by including face landmark prediction.


%Although great progress has been achieved, most methods simply hypothesize that human skeletons are mainly correlated with rhythm and beat and generating human skeletons based on only low-dimensional rhythm features, which limits their expressive capability.
%Early attempts to achieve this goal mainly focus on face region, and leave the main body parts like the torsos and the limbs ignored \cite{}.

%To improve the diversity of generated motion, we propose to incorporate the powerful large language model priors into existing audio-driven gesture generation pipeline.
%By aligning the speech features with linguistic representations, we are able to enhance understanding of the contextual nuances inherent in the spoken content.


To improve the diversity and expressiveness of the synthesized motions, we propose integrating powerful large language model (LLM) priors within our audio-driven gesture synthesis framework. Aligning speech features with linguistic representations bolsters our comprehension of the contextual nuances inherent within the spoken content.
%To improve the diversity and expressiveness of generated motions, we propose to integrate powerful large language model (LLM) priors within our audio-driven gesture synthesis framework. By aligning the speech features with linguistic representations, we enhance the understanding of the contextual nuances inherent in the spoken content.
%this paper introduces a novel perspective by viewing the co-gesture generation challenge as a language translation task, translating from verbal language to non-verbal bodily languages. We tackle this translation task within a diffusion-conditional framework, leveraging the prowess of large language models as a foundational prior.
%In response to the above limitations, in this paper, we propose a new perspective that views the co-gesture generation problem as a language translation problem from verbal language to non-verbal bodily language, where we address this translation problem in a diffusion-conditional framework with the help of large language models prior.
Specifically, our methodology first employs a pre-trained audio feature extractor to distill high-dimensional semantic information from the input speech, subsequently projecting these features into the latent space of large language models. %This step facilitates the alignment of speech features with linguistic representations. 
%Thereafter, these language-aligned features are fed into large language models to improve semantic comprehension. 
%By doing so, we improve understanding of the contextual nuances inherent in the spoken content.
% Finally, the enriched semantic features are sent into diffusion models as conditional inputs, guiding the creation of gestures. The integration of large language model priors empowers our system to synthesize gestures that demonstrate not only coherent with the accompanying audio but also a heightened level of stability and diversity.
Subsequently, these language-aligned features are utilized by large language models to augment semantic understanding. Finally, the enriched semantic features serve as conditional inputs to diffusion models, guiding the generation of gestures. The incorporation of large language model priors empowers our system with the capability to synthesize gestures that are not only coherent with the paired audio but also exhibit an elevated degree of stability and diversity.

% 0518
%Recent advancements in video generation technology have paved the way for rendering generated human gestures to photo-realistic and temporal-coherent videos within a zero-shot manner \cite{blattmann2023stable, hu2023animate}.
% 0518

%high-fidelity zero-shot human rendering, facilitated by the exploitation of pre-trained diffusion model priors. 
%Notably, Corona et al. \cite{corona2024vlogger} explore bridging the divide between general video synthesis techniques and the specific domain of audio-driven talking human video creation by adopting human video generation methods to render co-gesture generated skeletons.
%They achieved this by integrating human video generation methodologies to animate co-generated skeletal structures, marking a significant first step in synthesizing coherent and contextually appropriate gestures in response to audio cues.
% Recent success in video generation provides the possibility to achieve high-fidelity zero-shot rendering by leveraging the pre-trained diffusion model prior.
% Corona \textit{et. al} \cite{corona2024vlogger} make the first attempt to bridge the gap between video synthesis methods and audio-driven talking human video generation by adopting human video generation methods to render co-gesture generated skeletons.
%Integrating image region masks into video diffusion networks to make model aware of region segmentation encourages the model to deal with the specific property and improve the rendering stability and quality. However, there is no directly available human region mask in our case of audio-driven human synthesis.
%Moreover, existing human matting algorithms tend to generate sub-optimal temporal instable masks due to the lack of body gesture information. 

%Incorporating image region masks within video diffusion networks is a common strategy to improve the model's awareness of different image parts, thereby improving the consistency and stability of overall output \cite{yi2023generating, xue2023raphael}. Nevertheless, the absence of accessible human region masks prevents its application in the context of audio-driven human synthesis.
Integrating image region masks within diffusion networks is a common approach to enhance the model's recognition of distinct image segments, which improves the temporal consistency and stability of the synthesized output \cite{yi2023generating, xue2023raphael}. However, the unavailability of readily accessible human region masks prevents its implementation within audio-driven human synthesis tasks.
%Compounding this issue, prevailing human matting algorithms, which could potentially generate such masks, often yield suboptimal results with temporal instability. This deficiency is particularly pronounced due to the inadequacy of body gesture information in the algorithms, resulting in masks that fail to accurately capture the dynamic nature of human motion across frames.
To overcome this limitation, our solution integrates a Variational Autoencoder (VAE) \cite{kingma2014auto} network to dynamically generate human masks based on skeleton data, thus enabling mask guidance at inference time.
%and enhancing the accuracy of region segmentation.
These masks are further sent to a Mixture-of-Experts (MoE) module \cite{shazeer2017outrageously, fedus2022switch, xue2023raphael} we integrated into the diffusion rendering network, where each expert is guided by a dedicated region mask, empowering the model to distinguish varying image parts and improving the rendering stability and temporal consistency of talking video. 
Notably, the predicted masks achieve higher accuracy and stability than detected masks thanks to human motion information contained in skeleton data. %we also utilize these masks to train the MoE module. 
The enhancement in the quality of guided masks improves the training performance and ultimately contributes to increased realism and stability in the output videos.
%Complementarily, we train a Variational Autoencoder (VAE) \cite{kingma2014auto, rombach2022high} network to dynamically generate region masks based on human motion, thus enhancing the accuracy of region segmentation.
% Concurrently, we employ a Variational Autoencoder (VAE) network, which is trained to dynamically produce region masks informed by human skeletal data. This approach serves to enhance the accuracy of region segmentation and enables the real-time generation of masks during the inference phase, thereby augmenting the system's performance.
To ensure the generalization ability of our framework, we also present a large-scale High-definition Audio-Visual dataset (HDAV) containing 4023 identities with 2D human keypoint annotations and detail property labels.

In summary, our major contributions are as follows:
\begin{itemize}
    \item We present a framework designed for the one-shot generation of high-fidelity talking human videos, surpassing the performance of existing methods.
    \item We leverage the powerful large language model priors to guide cross-modal translation and elevate the diversity of gesture generation.
    \item We devise a mask-guided MoE module, which improves the overall visual rendering quality and stability by enhancing the distinction among varying human image regions.
    \item We release a large-scale dataset that significantly lowers the hurdles associated with training robust models for human video generation.%, thereby advancing the research frontier in this domain.
\end{itemize}
% 1) 
% 2) 
% 3) 
% 4) 

% In summary, our major contributions are as follows:
% 1) We present a framework to generate high-quality talking human video in a zero-shot manner which outperforms existing methods;
% 2) We propose to view co-gesture generation as a language translation problem and incorporate large language models prior to improving generation quality;
% 3) A mask-guided MoE module to improve overall rendering quality;
% 4) A large-scale dataset that significantly reduced the barrier to training robust human video generation models.

%, informed by the provided skeletal data, ensuring a spatially adaptive and nuanced rendering process.
%However, these methods typically render the whole image uniformly and ignore the specific properties of different image parts, which leads to artifact results.
%To address this limitation, we insert the Mixture-of-Experts mechanism into our diffusion rendering network, where each expert is guided by a specific region mask.
%We also train a vae network to generate region mask from skeletons at inference time.


%, and contextual appropriateness, thereby advancing the state-of-the-art in gesture synthesis.

% Specifically, we first adopt a pre-trained audio feature extractor to extract the high-dimensional semantic features of input speech and project these features to the latent space of large language models.
% Then, we send these language-like representations to large language models for improving semantic understanding and reasoning.
% After that, these semantic features are send to diffusion models as conditional signal to guide gesture generation.
% With the help of large language model prior, we are able to generate gestures that are not only coherent with input audio, but also own more breadth and depth.


% 1. two goals 
% audio to motion 

% low dimensional

% to high dimensional semantic

% search and find

% cross-modal 

% unify-modal


%Render
\begin{figure*}
    \centering
    \includegraphics[width = 1\textwidth]{img/overview9.jpg}
    \caption{The overall framework of LLM-Talker. Given a single portrait image with its driven audio, we first convert the audio input to human motion sequences based on large language model priors. Then, we render these motions to high-fidelity human videos through a U-net backbone, where a mask-guided Mixture-of-experts (MoE) module improves the rendering stability. Notably, we train a mask generation network to predict the human mask at inference time.}
    \label{fig:main}
\end{figure*}

